BachGAN: High-Resolution Image Synthesis from Salient Object Layout

We propose a new task towards more practical application for image generation - high-quality image synthesis from salient object layout. This new setting allows users to provide the layout of salient objects only (i.e., foreground bounding boxes and categories), and lets the model complete the drawing with an invented background and a matching foreground. Two main challenges spring from this new task: (i) how to generate fine-grained details and realistic textures without segmentation map input; and (ii) how to create a background and weave it seamlessly into standalone objects. To tackle this, we propose Background Hallucination Generative Adversarial Network (BachGAN), which first selects a set of segmentation maps from a large candidate pool via a background retrieval module, then encodes these candidate layouts via a background fusion module to hallucinate a suitable background for the given objects. By generating the hallucinated background representation dynamically, our model can synthesize high-resolution images with both photo-realistic foreground and integral background. Experiments on Cityscapes and ADE20K datasets demonstrate the advantage of BachGAN over existing methods, measured on both visual fidelity of generated images and visual alignment between output images and input layouts.

==> supp_concat.tex <==


%%%%%%%%% TITLE

% \title{Supplementary Material: BachGAN}
\begin{figure*}[t!]
  \centering
  \includegraphics[width = \textwidth]{./cityscapes.pdf}
  \caption{Additional examples of image synthesis results from different models on the Cityscapes dataset. }
  \label{fig:vis:city:app}
\end{figure*}


\begin{figure*}[t]
  \centering
  \includegraphics[width = 0.98\textwidth]{./ade20k_1_box.pdf}
  \caption{Additional examples of image synthesis results from different models on the ADE20K dataset. }
  \label{fig:vis:ade20:a}
\end{figure*}

\begin{figure*}[t]
  \centering
  \includegraphics[width = 0.98\textwidth]{./ade20k_2_box.pdf}
  \caption{Additional examples of image synthesis results from different models on the ADE20K dataset.}
  \label{fig:vis:ade20:b}
\end{figure*}

\begin{figure*}
  \centering
  \includegraphics[width = 0.98\textwidth]{./layout2img.pdf}
  \caption{Examples of image synthesis results from Layout2im on the Cityscapes datasets.}
  \label{fig:vis:layout2im}
\end{figure*}

\section{Additional Ablation Study}
%
In Table \ref{tab:size:bank:app}, we show additional results of models trained with memory banks of different size on both datasets. With half-sized memory banks, BachGAN still achieves good performance measured by FID scores. These results demonstrate that our model is not sensitive to this hyper-parameter. 

\begin{table}[h]
\centering
\begin{tabular}{c|c|c}
\hline 
Datasets  & Cityscapes & ADE20K \\
\hline
$\frac{1}{2} \times |\mathbf{B}|$ & 74.2 & 51.2 \\
\hline
$|\mathbf{B}|$ & 73.3 & 49.8\\
\hline
$2 \times |\mathbf{B}|$ & 72.5 & -\\
\hline
\end{tabular}
\caption{FID scores of BachGAN trained using different memory bank sizes on Cityscapes and ADE20K.}
\label{tab:size:bank:app}
\end{table}

\section{Additional Implementation Details}
\paragraph{Generator} The architecture of the generator follows the one used in~\cite{park2019semantic}, which consists of several SPADE Residual Blocks with nearest neighbor upsampling. We train the model on 8 V100 GPUs with synchronized BatchNorm. Instead of feeding the label map of object layout into each SPADE layer, we obtain the object layout with fine-grained background (or the fusion of several background segments), and take it as the input. 

\paragraph{Discriminator}
The architecture of the discriminator also follows the one used in SPADE ~\cite{park2019semantic} and pix2pixHD~\cite{wang2018high}, which
uses a multi-scale design with InstanceNorm (IN), and applies Spectral Norm to all the convolutional layers. Compared with them, the difference of our model is that the input includes both real images and the object layouts with hallucinated background.

\paragraph{Background Fusion Module}
As illustrated in Figure 2 and Section 3.3 of our main manuscript, the Background Fusion Module has 2 convolutional neural networks -- $\mathcal{F}$ and  $\mathcal{M}$.  Specifically, $\mathcal{F}$ is used for encoding the label maps, and $\mathcal{M}$ is used to process the fused feature of foreground layout and background segments. Both $\mathcal{F}$ and $\mathcal{M}$
include a $3 \times 3$ convolutional layer with $k$ convolutional filters and ReLU activation functions, where $k$ is $C_o+C_b$. 

\paragraph{Retrieval Time} The average time for calculating each $\text{IoU}_r$ is 4ms. In our paper, we compute all $\text{IoU}_r$ in a sequential way (one by one), which takes $\sim$20 seconds (for $|\mathbf{B}|$ = 5,000 maps).
This could be further improved by paralleling the computation.

\paragraph{Sequential Generation} In order to generate consistent images, we use the same retrieved semantic segmentation maps as the background inputs. In addition, the generation process is deterministic, which means no random noise is added to the training and testing stages.This property indicates that BachGAN can generate similar results for each object as long as they have the same layout.


\section{Additional Synthesized Images}
In Figure \ref{fig:vis:city:app}, \ref{fig:vis:ade20:a} and \ref{fig:vis:ade20:b}, we show additional synthesized images from the proposed method on the Cityscapes and ADK20K datasets, with comparisons to the baseline models. 
In Figure \ref{fig:vis:layout2im}, we show the generated images using Layout2im \cite{zhaobo2019layout2im} on Cityscapes. 

%\section{Additional Experimental Details}





